Timescales of Chaos in the Inner Solar System: Lyapunov Spectrum and Quasi-integrals of Motion

Numerical integrations of the Solar System reveal a remarkable stability of the orbits of the inner planets over billions of years, in spite of their chaotic variations characterized by a Lyapunov time of only 5 million years and the lack of integrals of motion able to constrain their dynamics. To open a window on such long-term behavior, we compute the entire Lyapunov spectrum of a forced secular model of the inner planets. We uncover a hierarchy of characteristic exponents that spans two orders of magnitude, manifesting a slow-fast dynamics with a broad separation of timescales. A systematic analysis of the Fourier harmonics of the Hamiltonian, based on computer algebra, reveals three symmetries that characterize the strongest resonances responsible for the orbital chaos. These symmetries are broken only by weak resonances, leading to the existence of quasi-integrals of motion that are shown to relate to the smallest Lyapunov exponents. A principal component analysis of the orbital solutions independently confirms that the quasi-integrals are among the slowest degrees of freedom of the dynamics. Strong evidence emerges that they effectively constrain the chaotic diffusion of the orbits, playing a crucial role in the statistical stability over the Solar System lifetime.

==> iss3_commands.tex <==
% Format statistical results with their bounds
\makeatletter
\newcommand{\raisemath}[1]{\mathpalette{\raiseboxmath{#1}}}
\newcommand{\raiseboxmath}[3]{\raisebox{#1}{$#2#3$}}
\makeatother
\newcommand{\stats}[3]{${#1}_{\raisemath{2pt}{\scriptscriptstyle #2}}^{\raisemath{0.5pt}{\scriptscriptstyle #3}}$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\g@addto@macro{\endtabular}{\rowfont{}}% Clear row font
\makeatother
\newcommand{\rowfonttype}{}% Current row font
\newcommand{\rowfont}[1]{% Set current row font
   \gdef\rowfonttype{#1}#1%
}
\newcolumntype{L}{>{\rowfonttype}l}

% Please keep new commands to a minimum, and use \newcommand not \def to avoid
% overwriting existing commands. Example:
%\newcommand{\pcm}{\,cm$^{-2}$}	% per cm-squared
\newcommand{\Poincare}{Poincar\'{e}}
\newcommand{\arcsecyr}{$^{\prime\prime} \,{\textrm{yr}}^{-1}$}
\newcommand{\arcsecyrtext}{${\textrm{arcsec yr}}^{-1}$}

\def\TRIP{\textsc{TRIP}}

\let\vec\boldsymbol
\def\E{\mathrm{E}}
\def\inc{\mathcal{I}}

\def\DOF{DOF}
\newcommand{\nomsol}{$\mathcal{S}$}
\newcommand{\lienomsol}{$\mathcal{S}^\prime$}

\newcommand{\subscript}[2]{#1_{\textnormal{\scriptsize #2}}}
\newcommand{\superscript}[2]{#1^{\textnormal{\scriptsize #2}}}

\newcommand{\Hsec}{\widehat{H}}
\newcommand{\Hiss}{\mathcal{H}}
\newcommand{\HLL}{\subscript{\Hsec}{LL}}

\newcommand{\out}[1]{\subscript{#1}{o}}

\newcommand{\gLL}{\subscript{g}{LL}}
\newcommand{\sLL}{\subscript{s}{LL}}
\newcommand{\vecomegaLL}{\subscript{\vec{\omega}}{LL}}

\newcommand{\vecu}{\vec{u}}
\newcommand{\vecv}{\vec{v}}

\newcommand{\Huv}{\mathbb{H}}

% \newcommand{\Chi}{X}
\newcommand{\Chi}{\mathfrak{X}}

\newcommand{\vecChi}{\vec{\Chi}}
\newcommand{\vecchi}{\vec{\chi}}
\newcommand{\vecPsi}{\vec{\Psi}}
\newcommand{\vecpsi}{\vec{\psi}}
\newcommand{\vecI}{\vec{I}}
\newcommand{\vectheta}{\vec{\theta}}
\newcommand{\veck}{\vec{k}}
\newcommand{\vecl}{\vec{\ell}}

\newcommand{\vecomegamean}{\overline{\vec{\omega}}}
\newcommand{\vecomegaout}{\out{\vec{\omega}}}

\newcommand{\fourcoeff}[3]{\widetilde{\Huv}_{#1}^{\vec{#2},\vec{#3}}}
\newcommand{\Ham}[1]{\Huv_{#1}}
\newcommand{\Hamstar}[1]{\Huv_{#1}^\star}
\newcommand{\lieham}{\Huv^\prime}
\newcommand{\Hamstart}{\Ham{6}}

\newcommand{\lieI}{\vecI^\prime}
\newcommand{\lietheta}{\vectheta^\prime}
\newcommand{\liePhi}{\vec{\Phi}^\prime}
\newcommand{\liephi}{\vec{\phi}^\prime}
\newcommand{\lieomega}{\vec{\omega}^\prime}
\newcommand{\lieomegamean}{\vec{\vecomegamean}^\prime}

\newcommand{\liefourcoeff}[2]{\widetilde{\Huv}_{2n}^{\prime \, \vec{#1},\vec{#2}}}

\newcommand{\vecp}{\vec{p}}
\newcommand{\vecvarphi}{\vec{\varphi}}
\newcommand{\vece}{\vec{e}}

\newcommand{\conj}[1]{\overline{#1}}
\newcommand{\lieChi}{\vec{\Chi}^\prime}
\newcommand{\liePsi}{\vec{\Psi}^\prime}

\def\F{\mathcal{F}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\newcommand{\lietransf}{\mathcal{L}}

\def\omegaell{\omega_\mathrm{ell}}
\def\omegahyp{\omega_\mathrm{hyp}}
\def\halfwidth{\Delta\omega}
\def\omegamean{\overline{\omega}}

\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\vecz}{\vec{z}}
\newcommand{\veczeta}{\vec{\zeta}}
\newcommand{\vecF}{\vec{F}}
\newcommand{\matM}{\mathbf{M}}
\newcommand{\matJ}{\mathbf{J}}
\newcommand{\matLambda}{\mathbf{\Lambda}}

% \def\simpleH{\widetilde{\Huv}_4}
\newcommand{\simpleH}[1]{\Huv_{#1}^\bullet}

\def\O{\mathcal{O}}
\newcommand{\vecalpha}{\vec{\alpha}}
\newcommand{\vecbeta}{\vec{\beta}}
\newcommand{\vecq}{\vec{q}}
\newcommand{\Span}{\operatorname{span}}

\def\C{\mathcal{C}}

\newcommand{\veckappa}{\vec{\kappa}}
\newcommand{\vecke}{\superscript{\veck}{ecc}}
\newcommand{\vecki}{\superscript{\veck}{inc}}

\newcommand{\inn}[1]{\subscript{#1}{i}}
\newcommand{\vecomegainn}{\inn{\vec{\omega}}}

\newcommand{\vecgamma}{\vec{\gamma}}
\DeclareBoldMathCommand\bgamma{\gamma}

\newcommand{\Cinc}{\subscript{\mathcal{C}}{inc}}
\newcommand{\Cecc}{\subscript{\mathcal{C}}{ecc}}

\newcommand{\Cinchat}{\subscript{\widehat{\mathcal{C}}}{inc}}

\def\R{\mathcal{R}}

\newcommand{\LL}[1]{#1_{\scaleto{\textsc{LL}}{4pt}}}
\newcommand{\mat}[1]{\mathbf{#1}}

